Learning to Cluster via Same-Cluster Queries

We study the problem of learning to cluster data points using an oracle which can answer same-cluster queries. Different from previous approaches, we do not assume that the total number of clusters is known at the beginning and do not require that the true clusters are consistent with a predefined objective function such as the K-means. These relaxations are critical from the practical perspective and, meanwhile, make the problem more challenging. We propose two algorithms with provable theoretical guarantees and verify their effectiveness via an extensive set of experiments on both synthetic and real-world data.

==> improved_analysis.tex <==
\section{Improved Algorithm}\label{sec:main_analysis}

The improved algorithm is presented in Algorithm~\ref{alg:main} and this section is devoted to its analysis. 


==> more-exp.tex <==
\section{Additional Experiments}
\label{sec:experiment}

\noindent{\bf Synthetic Data.} 
For synthetic datasets, we generate $n$ points that belong to $K$ clusters in the $d$-dimensional Euclidean space. Since in the real world the cluster sizes typically follow a {\em power-law} distribution, we assign to each cluster a random size drawn from the widely used {\em Zipf distribution}, which has the density function $f(x)\propto x^{-\alpha}$, where $x$ is the size of the cluster and $\alpha$ a parameter controlling the skewness of the dataset. We then choose a center $\mu_i$ for each cluster $i\in [K]$ in a manner to be specified later and generate the points in the cluster from the multivariate Gaussian distribution $N(\mu_i, \sigma^2 I_d)$, where $I_d$ denotes the $d \times d$ identity matrix.

Now we specify how to choose the centers. In practice, clusters in the dataset are not always well separated; there could be clusters whose centers are close to each other.  We thus use an additional parameter $p$ to characterize this phenomenon.  In the default setting of $p = 0$, all centers of the $K$ clusters are drawn uniformly at random from $[0, b]^d$.  When $p > 0$, we first partition the clusters into groups as follows: Think of each cluster as a node. For each pair of clusters, with probability $p$ we add an edge between the two nodes.  Each connected component of the resulting graph forms a group.  Next, for each group of clusters, we pick a random cluster and choose its center $\mu$ uniformly at random in $[0, b]^d$. For each of the remaining clusters in the group, we choose its center uniformly at random in the neighborhood of radius $\rho$ centered at $\mu$.

We use the following set of parameters as the default setting in our synthetic datasets:
$n=10^6$, $K=100$, $\alpha=2.5$, $\sigma=0.3$, $b=5$, $d=10$ and $\rho=0.1$.

In addition, we simulate the cluster separation property by a collision probability $p$,
which is the probability that a cluster has its center very close to another
randomly chosen cluster. 
We consider three values of $p\in \{0,0.1,0.3\}$ to simulate no collision, low collision and high collision scenarios. 
The higher the collision probability is, the more difficult it is for the $D^2$-sampling to recover clusters. 


\vspace{2mm}

\noindent{\bf Query Complexity.}
The results for synthetic dataset are plotted in Figure~\ref{fig:synthetic}. We also observe that \improved\ performs better than \baseline, a phenomenon more pronounced in the more difficult case of $p=0.3$ for the synthetic dataset and in the \kdd\ dataset. Only in the \shuttle\ dataset, they have almost the same performance in the fixed-recovery setting.

Tables~\ref{tab:sim-query} and \ref{tab:sim-cluster} present the statistics of the performance of three tested algorithms on the synthetic datasets, in the fixed-budget and fixed-recovery setting, respectively. Tables~\ref{tab:shuttle} and \ref{tab:kdd} present the statistics of the performance of three tested algorithms on two real-world datasets \shuttle\ and \kdd\ respectively.

It is clear that \baseline\ and \improved\ significantly outperform \uniform\  in all cases. Take \kdd\ dataset for example, we observe that with $10^5$ query budget \uniform\ recovers $10$ clusters while \baseline\ and \improved\ recover around $18$ clusters.  In order to recover $16$ clusters, \uniform\ requires $200,000$ queries per cluster, while \baseline\ and \improved\ only requires no more than $2,500$ queries per cluster.  Even on small datasets such as \shuttle, \uniform\ needs about twice amount of queries to recover all clusters compared with \baseline\ and \improved.  We also observe that \improved\ performs slightly better than \baseline.

On synthetic datasets, one can see that higher collision probability $p$ makes clustering more difficult for all algorithms.  Given a query budget of $2 \times 10^5$, \baseline\ and \improved\ can recover about $70$ clusters when $p = 0$ (no collision),  but only about $60$ clusters when $p = 0.3$. 

%\begin{figure}[th!]
%\centering
%\begin{minipage}[d]{0.325\linewidth}
%\begin{overpic}[width=\textwidth,percent]{./figs/a25}
%	\put(13,65){\scriptsize $p=0$}
%\end{overpic}
%\end{minipage}
%\hfill
%\begin{minipage}[d]{0.325\linewidth}
%\begin{overpic}[width=\textwidth,percent]{./figs/p1}
%	\put(13,63){\scriptsize $p=0.1$}
%\end{overpic}
%\end{minipage}
%\begin{minipage}[d]{0.325\linewidth}
%\begin{overpic}[width=\textwidth,percent]{./figs/p3}
%	\put(13,63){\scriptsize $p=0.3$}
%\end{overpic}
%\end{minipage}

%\begin{minipage}[d]{0.325\linewidth}
%\begin{overpic}[width=\textwidth,percent]{./figs/c_a25}
%	\put(13,65){\scriptsize $p=0$}
%\end{overpic}
%\end{minipage}
%\hfill
%\begin{minipage}[d]{0.325\linewidth}
%\begin{overpic}[width=\textwidth,percent]{./figs/c_p1}
%	\put(13,63){\scriptsize $p=0.1$}
%\end{overpic}
%\end{minipage}
%\hfill
%\begin{minipage}[d]{0.325\linewidth}
%\begin{overpic}[width=\textwidth,percent]{./figs/c_p3}
%	\put(13,63){\scriptsize $p=0.3$}
%\end{overpic}
%\end{minipage}
%\vspace{-0.5em}
%\caption{Performance comparison on synthetic datasets. The top row is the fixed-budget case and the bottom row is the fixed-recovery case.}
%\label{fig:synthetic}
%\end{figure}


% From ICML exp.tex



\vspace{2mm}

\noindent{\bf Center Approximation.} \
For measuring the quality of outputted approximate centers, we run the three algorithms in the fixed-recovery case.  We report the median error of all recovered clusters on synthetic, \shuttle\ and \kdd\ datasets in Tables~\ref{tab:sim-error}, \ref{tab:shuttle-error}, and \ref{tab:kdd-error}, respectively.  We observe that all error rates are below $10\%$: The error rates are about 9\% on the synthetic datasets and are about 5\% on the two real-world datasets. There is no significant difference between the error rates of different algorithms; the maximum difference is no more than 2\%.  Generally speaking, all tested algorithms achieve satisfactory center approximations.




\vspace{2mm}

\noindent{\bf Time and Rounds.}  Finally we compare \baseline\ and \improved\ on running time and round usage.  The results are presented in Figure~\ref{fig:sim-time}, \ref{fig:sim-round}, \ref{fig:shuttle-time}, and \ref{fig:kdd-time}.  It is clear that \improved\ uses less time and fewer rounds than \baseline.  The only exception is the \shuttle\ dataset, where the performance of \baseline\ and \improved\ are almost the same; this may be because the number of clusters in \shuttle\ is too small ($7$ in total) for the algorithms to make any difference.







==> notations.tex <==
\begin{table}[!tb]
\caption{Notations}\label{tab:notations}
\begin{tabular}{|l|l||l|l|}
\hline
$X$ & set of input points & \multirow{2}{*}{$W$} & set of indices of clusters to\\
\cline{1-2}
$r$ & index of the round & & recover \\
\hline
$I$ & set of indices of recovered clusters so far & \multirow{2}{*}{$K$} & total number of recovered  \\
\cline{1-2}
$k$ & number of recovered clusters so far & &  clusters at the end\\
\hline
\multirow{2}{*}{$Q$} & set of indices of newly discovered clusters & \multirow{2}{*}{$L$} & total number of discovered \\ 
& in the current round & & clusters at the end \\
\hline
\multirow{2}{*}{$S$} & multiset of samples. Each sample has the form of & \multirow{3}{*}{$S_j$} & multiset of uniform samples in \\
    & $(x,i)$, where $x$ is the point and $i$ the cluster index. & & cluster $j$ returned by rejection  \\
\cline{1-2}
$x_j^\ast$ & reference point in cluster $j$ for rejection sampling & & sampling. Note that $S\neq \bigcup_j S_j$.\\
\hline
\end{tabular}
\end{table}

